An Open-System Quantum Simulator with Trapped Ions

The control of quantum systems is of fundamental scientific interest and promises powerful applications and technologies. Impressive progress has been achieved in isolating the systems from the environment and coherently controlling their dynamics, as demonstrated by the creation and manipulation of entanglement in various physical systems. However, for open quantum systems, engineering the dynamics of many particles by a controlled coupling to an environment remains largely unexplored. Here we report the first realization of a toolbox for simulating an open quantum system with up to five qubits. Using a quantum computing architecture with trapped ions, we combine multi-qubit gates with optical pumping to implement coherent operations and dissipative processes. We illustrate this engineering by the dissipative preparation of entangled states, the simulation of coherent many-body spin interactions and the quantum non-demolition measurement of multi-qubit observables. By adding controlled dissipation to coherent operations, this work offers novel prospects for open-system quantum simulation and computation.

==> includes/sub-bsc.tex <==

\subsection{Implemented Kraus maps}

The Bell state $\ket{\Psi^-}$ is not only uniquely determined as the
simultaneous eigenstate with eigenvalue -1 of the two stabilizer operators
$X_1X_2$ and $Z_1Z_2$ (as mentioned in the text), but also by $X_1X_2$ and
$Y_1Y_2$. In the experiment, we implemented cooling into $\ket{\Psi^-}$ by
engineering the two Kraus maps $\rho_S \mapsto E_1\rho_S E_1^\dagger +
E_2\rho_S E_2^\dagger$ and $\rho_S \mapsto E'_1\rho_S {E'_1}^{\dagger} +
E'_2\rho_S {E'_2}^{\dagger}$, where
\begin{align}
%\label{eq:XXKrausMap}
E_{1} & = \sqrt{p} \, Y_1 \frac{1}{2} \left(1 + X_1X_2 \right), \nonumber \\
E_{2} & = \frac{1}{2} \left( 1 - X_1X_2 \right) +  \sqrt{1-p} \,\frac{1}{2} \left( 1 + X_1X_2 \right),\nonumber\\
%\label{eq:YYKrausMaps}
E'_{1} & = \sqrt{p} \, X_1 \frac{1}{2} \left(1 +Y_1Y_2 \right), \nonumber \\
E'_{2} & =  \frac{1}{2} \left( 1 - Y_1Y_2 \right) +  \sqrt{1-p} \,\frac{1}{2} \left( 1 + Y_1Y_2 \right),\nonumber
\end{align}
which generate pumping into the -1 eigenspaces of $X_1X_2$ and $Y_1Y_2$
(instead of pumping into the eigenspaces of $X_1X_2$ and $Z_1Z_2$ as explained
in Box~1 of the main text). The reason for pumping into the eigenspaces of
$X_1X_2$ and $Y_1Y_2$ is that the mapping and unmapping steps, shown as (i) and
(iii) in Box 1, are realized by a single MS gate $U_{X^2}(\pi/2)$ and
$U_{Y^2}(\pi/2)$, respectively.

\subsection{Circuit decomposition}

The map for pumping into the -1 eigenspace of $X_1X_2$ was implemented by the
unitary 
\begin{equation}
U_{X^2(\pi/2)} \,C(p) \, U_{X^2(\pi/2)}
\end{equation}
(corresponding to steps (i) - (iii) in Box~1) followed by an optical pumping of
the ancilla qubit to $\ket{1}$.  Here, the two-qubit controlled gate is
\begin{eqnarray}
C(p) & = & \ket{0}\bra{0}_0 \otimes \exp(i\alpha Z_1) + \ket{1}\bra{1}_0
\otimes \openone \nonumber \\ & = & \exp \left[ \frac{1}{2} (1+ Z_0) i \alpha Z_1
  \right] \nonumber \\ & = & U_{Z_1} (-\alpha)\, U_{Y}(\pi/2)\,
U_{X^2}^{(0,1)}(-\alpha) \,U_{Y}(-\pi/2)
\end{eqnarray}
where $U_{X^2}^{(0,1)}(-\alpha) = \exp(i(\alpha/2) X_0 X_1)$ denotes an MS gate
acting only on the ancilla and the first system qubit. This two-qubit MS gate
operation was implemented in the experiment by the use of refocusing
techniques~\citep{nebendahl-pra-79-012312}.  In more detail, the gate
$U_{X^2}^{(0,1)}$ was realized by interspersing two of the available
three-qubit MS gate operations with single-ion light shifts on the second
system qubit which induces a $\pi$-phase shift between the qubit states.
Alternatively, this refocusing could be avoided, and the sequences further
simplified, by hiding the population of individual ions (here the second system
ion) which are not supposed to participate in collective coherent operations in
electronic levels decoupled from the driving laser excitation. More details on
how to systematically decompose Kraus maps into the experimentally available
ion-trap gate operations, in particular the multi-ion MS entangling gate, can
be found in~\cite{mueller-2010}.

The circuit decompositions for the experimental implementation of the two maps
are shown in Fig.~\ref{fig:bsc-circuits}.  We note that the circuits have
been simplified at the expense of implementing in addition in each dissipative
map a flip operation $Y_1Y_2$ on the two system qubits. However, as this
additional unitary corresponds to one of the stabilizers into whose -1
eigenspace cooling is performed, this does not interfere with the cooling
dynamics.

Cooling with unit pumping probability $p=1$ corresponds to $\alpha = \pi/2$,
whereas $p=0.5$ is realized with by setting $\alpha = \pi/4$. In the
experiment, the "fundamental" MS gate was calibrated to implement
$U_{X^2}(\alpha/2)$. The fully entangling operation $U_{X^2}(\pi/2)$ at the
beginning and the end of the sequence Fig.~\ref{fig:bsc-circuits}a was then
implemented by applying the $U_{X^2}(\alpha/2)$ operation twice (for $p=1$) or
four times (for $p=0.5$).  The fully entangling operations $U_{Y^2}(\pi/2)$ in
Fig.~\ref{fig:bsc-circuits}b were implemented by two- and four-fold application
of the "fundamental" MS gate with a shifted optical phase of the driving laser
(cf.~Section 2 in the main text).

\begin{figure}[h!]
\begin{center}
\iffigs \includegraphics{figures/figureSI1}\fi
\end{center}
\caption{\label{fig:bsc-circuits} \textbf{Experimental sequences for Bell-state
    cooling.} Pumping into the eigenspaces of eigenvalue -1 of $X_1X_2$ (circuit \textbf{a,}) and
  $Y_1Y_2$ (circuit \textbf{b,}) occurs with a probability $p$ in each step, where $\sin^2\alpha =
  p$.}
\end{figure}

\subsection{Additional data}

The initially mixed state was prepared with a fidelity of F=99.6(3)\% with
respect to the ideal state $\frac{1}{4}\openone_{4\times4}$.

Physical process matrices were reconstructed with maximum likelihood
techniques~\citep{jezek-pra-68-012305}.  An error analysis was carried out via
Monte Carlo simulations over the multinomially distributed measurement outcomes
of the state and process tomography.  For each process and state, 200 Monte
Carlo samples were generated and reconstructed via maximum-likelihood
estimation.

